Equivalence-based Security for Querying Encrypted Databases: Theory and Application to Privacy Policy Audits

Motivated by the problem of simultaneously preserving confidentiality and usability of data outsourced to third-party clouds, we present two different database encryption schemes that largely hide data but reveal enough information to support a wide-range of relational queries. We provide a security definition for database encryption that captures confidentiality based on a notion of equivalence of databases from the adversary's perspective. As a specific application, we adapt an existing algorithm for finding violations of privacy policies to run on logs encrypted under our schemes and observe low to moderate overheads.

==> correctness.tex <==
In this section, we will prove the functional correctness of \ereduce in the \dt 
instance of our framework. %The proof of correctness in \kh is similar. 
In \dt, \ereduce does not require any hash adjustments  
and hence we will consider $\vec{\Delta} = \emptyset$. Additionally, the $\Psi$ function 
in the $\textsc{R-P}$ case 
does not require any hash adjustments and instead 
just grounds the variables in the input predicate $\pred{p}$ 
by applying the substitution $\sigma$. 

\paragraph*{Alternate representation of plaintext audit log} As noted earlier, 
a plaintext audit log is a database with several tables where an encrypted audit log is a pair $\langle e\db, e\cT\rangle$ 
where $e\db$ is the encrypted audit log and $e\cT$ is the \DOPE data structure. However, for sake of presentation of this 
section only, we consider that even for the plaintext audit log we have a corresponding \DOPE data structure where each 
of the individual time-stamp is a plaintext value rather than an encrypted value. Hence, in this section, we will consider a 
plaintext audit log $\cL$ to be a pair $\langle\db, \cT\rangle$.  

\paragraph*{Substitution}
Given a set of variables \var, a database schema \cS, and a  log $\cL$, 
\emph{a substitution} $\sigma$ is a sequence of tuples of form $\langle x, v, t, c\rangle$ where 
$x\in\var$, $v$ is a value drawn from table $t$'s $c$th column of the log \cL. 
For simplicity we do not explicitly mention the set of variables, database schema, and the log 
when they are clear from the context or are not important.  
%Given a substitution $\sigma$, we call each tuple of form $\langle x, v, t, c\rangle\in\sigma$, 
%the \emph{substitution element} of $\sigma$. Each substitution element $\langle x, v, t, c\rangle$ signifies 
%that the variable $x$ is mapped to the value $v$ where $v$ is obtained from the $c$th column of table $t$. 
%The $(t,c)$ pair can be viewed as the taint label of the data $v$ signifying the source of the data. 
We call a substitution $\sigma$ \emph{well-formed} if there does not exist two different 
tuples $\langle x, v_1,t_1,c_1\rangle, \langle y, v_2,t_2,c_2\rangle\in \sigma$ such that $x=y$. In the 
sequel, we refer to a well-formed substitutions as just substitutions. 

 For a given substitution $\sigma$, we call the set of variables 
for which there are values according to $\sigma$, the set of \emph{mapped variables} and it can be defined as follows. 
\[
\pred{MappedVariables}(\sigma)=\{x\mid\exists v, t, c.\langle x,v,t,c\rangle\in\sigma\}
\]  
Given two substitutions $\sigma_1$ and $\sigma_2$, we say $\sigma_1$ is \emph{consistent} with $\sigma_2$ if and only if 
$\pred{MappedVariables}(\sigma_1)\supseteq \pred{MappedVariables}(\sigma_2)$ and 
$\forall x\in\pred{MappedVariables}(\sigma_2),\exists v,t,c. \langle x, v, t, c\rangle\in\sigma_1 \wedge 
\langle x, v, t, c\rangle\in\sigma_2$. 

Given a substitution $\sigma$, the source of the mapped variables of $\sigma$ (denoted by $\pred{Source}(\sigma)$) is 
defined as follows.  
\[
\pred{Source}(\sigma) = \{\langle x, t, c\rangle\mid \exists v.\langle x, v , t ,c \rangle\in \sigma\}
\]  
\paragraph*{Column equivalence class} 
Given any database schema \cS and a equality scheme \escheme, a \emph{column equivalence class} $E$ is a set of columns of form 
$\langle t, cl\rangle$ in which $t$ represents a table in \cS and $cl$ represents a column 
position in table $t$. We can uniquely identify any column in \cS with a corresponding  pair $\langle t, cl\rangle$. 
All columns in a equivalence class are deterministically encrypted with the same encryption key in \dt.    
Given a equality scheme \escheme, any database schema \cS we can find all the equivalence classes of columns in the following 
way. We create an undirected graph with all columns in \cS as nodes. For each tuple $\langle t_1, cl_1, t_2, cl_2\rangle$ 
we add an edge between the columns $\langle t_1, c_1\rangle$ and $\langle t_2, c_2\rangle$. Then we find the connected components 
in the resulting graph. Each connected component forms a column equivalent class. 

Given any database schema \cS, any equality scheme \escheme, any database \db with scheme \cS, 
any substitution $\sigma$, 
a set of column equivalence class $E=\{E_i\}_{i=1}^n$ obtained from \escheme, 
a set of injective functions $F=\{f_i\}_{i=1}^n$ where $f_i$'s domain 
comprises of the values in \cL which corresponds to the columns in equivalence class $E_i$, 
$F(\sigma)$ is defined in the following way: 
$F(\sigma)=\{\langle x, f_m(v), t, c\rangle\mid \langle x, v, t, c\rangle\in \sigma \wedge \langle t, c\rangle\in E_m\}$. 
The above definition can be generalized easily for a set of substitutions $\Sigma$ by applying $F$ on each substitution in $\Sigma$. 
We can also define application of $F$ over a plaintext policy $\policy$ by replacing each constant $c$ appearing in the policy 
predicate $\pred{p}$'s argument position $a$ by the value $f(c)$ where $f\in F$ is the corresponding injective function 
of the equivalence class of  predicate $\pred{p}$'s argument position $a$. We can also apply $F$ to the \cL in the similar fashion. 
%Special care should be given to applying $F$ to  $\cT$ \DOPE data structure of the plaintext log. The domain 
%of the corresponding injective function $f$ of the \DOPE data structure also contains the additional time-stamps  
%in \cT.  




For the following discussion, we require an auxiliary function $\pred{inputVar}(\cdot)$ 
which takes as argument a predicate and returns all the variables in its input argument positions. 
It can be defined as follows: 
$\pred{inputVar}(\pred{p}(t_1,\ldots,t_n)) = \{t_l\mid 1\leq l \leq \arity{\pred{p}} \wedge t_l\in\var \wedge l\in I(\pred{p})\}$.
The following claim is reasonable as \ereduce (\sathat) uses \sat as a black-box and for the database representation (consequently \DOPE data structure) 
the claim only assumes the correctness of the DBMS (resp., \DOPE data structure).   
\begin{claim}[\sat correctness]\label{claim:satCorrectness}
For any predicate $\pred{p}(\vec{t})$ such that 
there exists $\inp$, \outp, and $\mymap$ so that 
$\inp\nsat\pred{p}(t_1,\ldots,t_n):\langle \outp, \mymap\rangle$, 
for any schema \cS, for any plaintext log $\cL=\langle \db, \cT\rangle$, 
for all substitution $\sigma$ such that 
$\pred{MappedVariables}(\sigma)\supseteq \pred{inputVar}(\pred{p}(\vec{t}))$ and $\pred{Source}(\sigma)\supseteq \inp$, 
for all equality scheme \escheme and 
the set of column equivalence classes $E=\{E_i\}_{i=1}^n$ obtained from \escheme, for all injective function 
set $F =\{f_i\}_{i=1}^n$ where $f_i$'s domain contains all values in the equivalent class $E_i$, 
if $\sat(\cL,\pred{p}(\vec{t}),\emptyset,\sigma)\Downarrow\Sigma$ where each element of $\Sigma$ is consistent with $\sigma$ then 
$\sat(F(\cL),F(\pred{p}(\vec{t})),\emptyset,F(\sigma))\Downarrow F(\Sigma)$ where each element of $F(\Sigma)$ is consistent with $F(\sigma)$.  
\end{claim}
%\begin{proof}
%\textbf{Case} $\pred{p}(\vec{t}) = \pred{timeOrder}(x_1^+, d_1^+, x_2^+, d_2^+)$: 
%We know that all argument positions of \pred{timeOrder} are input argument positions. 
%Without loss of generality let us consider $x_1$ and $x_2$ to be variables. 
%From mode checking judgement \textsc{G-PRED} and from the premise we know that, 
%$x_1, x_2\in\pred{MappedVariables}(\sigma)$. Let us consider that for concrete 
%values $v_1$ and $v_2$ for $x_1$ and $x_2$, respectively, the above predicate holds 
%and 
%as none of the argument position is 
%output argument position
%\sat will return $\Sigma = \{\sigma\}$. We will now show that 
%$\sat(F(\cL),F(\pred{p}(\vec{t})),\emptyset,F(\sigma))\Downarrow F(\Sigma)$
%where $F(\Sigma) = \{F(\sigma)\}$. 

%From $\mathcal{A}$ we know that all argument positions of \pred{timeOrder} are in the same 
%equivalence class $E_i\in E$. 
%From the construction of \mymap in the \textsc{G-PRED} judgement, we know that $\langle t_1, c_1\rangle$ 
%and $\langle t_2, c_2\rangle$ are also in the equivalence class $E_i$ where $\exists v_1, v_2. 
%\langle x_1, v_1, t_1, c_1\rangle\in\sigma \wedge \langle x_2, v_2, t_2, c_2\rangle\in\sigma$. This implies 
%that they fall under the same injective function $f_i$. From the application of $f_i$ in $\sigma$, $\cT$ and from correctness of \cT, 
%we can say that $\pred{timeOrder}(f_i(v_1), f_i(d_1), f_i(v_2), f_i(d_2))$ holds. As none of the argument position is 
%output argument position \sat will return $\{f_i(\sigma)\}$.       

%\textbf{Case} $\pred{p}(\vec{t}) \neq \pred{timeOrder}(x_1^+, d_1^+, x_2^+, d_2^+)$: 
%From mode checking judgement \textsc{G-PRED} and from the premise we know that, 
%for all variables $x$ in the input argument position of \pred{p},    
%$x\in\pred{MappedVariables}(\sigma)$. From the premise ($\pred{Source}(\sigma)\supseteq \inp$) 
%and the construction of \mymap in \textsc{G-PRED}, for each variable $x$ in argument position $j$ ($1\leq j \leq \arity{\pred{p}}$) of 
%\pred{p}, we can say $\langle p, j\rangle$ and $\langle t, c\rangle$ are in the same equivalence class where 
%$\exists v. \langle x , v , t, c \rangle\in\sigma$. 
%As $\sat(\cL,\pred{p}(\vec{t}),\emptyset,\sigma)\Downarrow\Sigma$,  
%from the application of $F$ in \cL,  $\pred{p}(\vec{t})$, and $\sigma$, and 
%$F$ being an injective function set,  we have 
%$\sat(F(\cL),F(\pred{p}(\vec{t})),\emptyset,F(\sigma))\Downarrow F(\Sigma)$. 

%\end{proof} 



\begin{lemma}[Functional correctness of \sathat]\label{lemma:correctnessSathat}
For any formula $g$  such that there exists $\inp$, \outp, and $\mymap$ so that 
$\inp\nsat g:\langle\outp,\mymap\rangle$, for any schema \cS, for any plaintext log $\cL=\langle \db, \cT\rangle$, 
for all substitution $\sigma$ such that $\pred{MappedVariables}(\sigma)\supseteq \pred{FE}(\inp)$ and $\pred{Source}(\sigma)\supseteq\inp$, 
for all equality scheme \escheme  and 
the set of column equivalence classes $E=\{E_i\}_{i=1}^n$ obtained from \escheme, for all injective function 
set $F =\{f_i\}_{i=1}^n$ where $f_i$'s domain contains all values in the equivalent class $E_i$, 
if $\sathat(\cL,g,\emptyset,\sigma)\Downarrow\Sigma$ where each substitution in $\Sigma$ is consistent with $\sigma$ then 
$\sathat(F(\cL),F(g),\emptyset,F(\sigma))\Downarrow F(\Sigma)$ where each substitution in $F(\Sigma)$ is consistent with $F(\sigma)$.  
\end{lemma}
\begin{proof} Induction on the structure of the formula. 

\textbf{Case} $g = \pred{p}(\vec{t})$: This follows from Claim~\ref{claim:satCorrectness}. 

\textbf{Case} $g = g_1 \vee g_2$: From the definition of \sathat we know that, 
$\sathat(\cL,g_1\vee g_2,\emptyset,\sigma)\Downarrow \Sigma_1\cup\Sigma_2$ 
if and only if $\sathat(\cL,g_1,\emptyset,\sigma)\Downarrow \Sigma_1$ 
$\sathat(\cL,g_2,\emptyset,\sigma)\Downarrow \Sigma_2$. From induction hypothesis, 
we have $\sathat(F(\cL),F(g_1),\emptyset,F(\sigma))\Downarrow F(\Sigma_1)$ 
and $\sathat(F(\cL),F(g_2),\emptyset,F(\sigma))\Downarrow F(\Sigma_2)$. 
As $F(\Sigma_1\cup\Sigma_2) = F(\Sigma_1) \cup F(\Sigma_2)$, we have 
$\sathat(F(\cL),F(g_1\vee g_2),\emptyset,F(\sigma))\Downarrow F(\Sigma_1\cup\Sigma_2)$. 

\textbf{Case} $g = \exists x.g$: From the definition of \sathat we know that, 
$\sathat(\cL, \exists x.g,\emptyset,\sigma)\Downarrow \Sigma\setminus\{x\}$ if and only if 
$\sathat(\cL,g,\emptyset,\sigma)\Downarrow \Sigma$. As we have $\sathat(\cL,g,\emptyset,\sigma)\Downarrow \Sigma$ 
and from inductive hypothesis we have, 
$\sathat(F(\cL),F(g),\emptyset,F(\sigma))\Downarrow F(\Sigma)$. 
As $F(\Sigma)\setminus \{x\} = F(\Sigma\setminus\{x\})$, we have 
$\sathat(F(\cL), F(\exists x.g),\emptyset,F(\sigma))\Downarrow F(\Sigma\setminus\{x\})$. 

The rest of the cases are similar. 
\end{proof} 

\begin{lemma}[Functional correctness of \ereduce]\label{lemma:correctnessReduce}
For any policy \policy such that there exists $\inp$ and $\mymap$ so that 
$\inp\nsat\policy:\mymap$, for any schema \cS, for any plaintext log $\cL=\langle \db, \cT\rangle$, 
for all substitution $\sigma$ such that $\pred{MappedVariables}(\sigma)\supseteq \pred{FE}(\inp)$ and $\pred{Source}(\sigma)\supseteq\inp$, for all equality scheme \escheme 
and 
the set of column equivalence classes $E=\{E_i\}_{i=1}^n$ obtained from \escheme, for all injective function 
set $F =\{f_i\}_{i=1}^n$ where $f_i$'s domain contains all values in the equivalent class $E_i$, 
if $\ereduce(\cL,\policy,\emptyset,\sigma)\Downarrow\psi$ then 
$\ereduce(F(\cL),F(\policy),\emptyset,F(\sigma))\Downarrow F(\psi)$.  
\end{lemma}
\begin{proof}Induction on the structure of the formula. 

\textbf{Case} $\policy = \pred{p}(\vec{t})$: 
From mode checking judgement \textsc{R-P} and from the premise we know that, 
for all variables $x$ in the input argument position of \pred{p},    
$x\in\pred{MappedVariables}(\sigma)$. From the premise ($\pred{Source}(\sigma)\supseteq \inp$) 
and the construction of \mymap in \textsc{R-P}, for each variable $x$ in argument position $j$ ($1\leq j \leq \arity{\pred{p}}$) of 
\pred{p}, we can say $\langle p, j\rangle$ and $\langle t, c\rangle$ are in the same equivalence class where 
$\exists v. \langle x , v , t, c \rangle\in\sigma$. 

From the application of $F$ in \cL,  $\pred{p}(\vec{t})$, and $\sigma$, and 
$F$ being an injective function set, 
we have the following: 
(i) If $\cL(\pred{p}(\vec{t}))\sigma = \top$, then $F(\cL)(F(\pred{p}(\vec{t})))F(\sigma) = \top$. 
(ii) If $\cL(\pred{p}(\vec{t}))\sigma = \bot$, then $F(\cL)(F(\pred{p}(\vec{t})))F(\sigma) = \bot$.
(iii) If $\cL(\pred{p}(\vec{t}))\sigma = \mathsf{uu}$, then $F(\cL)(F(\pred{p}(\vec{t})))F(\sigma) = \mathsf{uu}$. 
Thus, if $\ereduce(\cL, \pred{p}(\vec{t}),\emptyset,\sigma)\Downarrow P$ 
then $\ereduce(F(\cL), F(\pred{p}(\vec{t})),\emptyset,F(\sigma))\Downarrow F(P)$. 

\textbf{Case} $\policy = \policy_1\wedge \policy_2$: 
From the definition of \ereduce, if $\ereduce(\cL,\policy_1\wedge\policy_2,\emptyset,\sigma)\Downarrow \psi$ 
then we have $\ereduce(\cL,\policy_1,\emptyset,\sigma)\Downarrow \policy'_1$, $\ereduce(\cL,\policy_2,\emptyset,\sigma)\Downarrow \policy'_2$, 
and $\psi\leftarrow\policy'_1\wedge\policy'_2$. As $\ereduce(\cL,\policy_1,\emptyset,\sigma)\Downarrow \policy'_1$ from induction 
hypothesis we have $\ereduce(F(\cL),F(\policy_1),\emptyset,F(\sigma))\Downarrow F(\policy'_1)$. Similarly we have 
$\ereduce(F(\cL),F(\policy_2),\emptyset,F(\sigma))\Downarrow F(\policy'_2)$. As $F(\policy'_1) \wedge F(\policy'_2) = F(\policy'_1 \wedge \policy'_2)$, 
we have $\ereduce(F(\cL),F(\policy_1\wedge\policy_2),\emptyset,F(\sigma))\Downarrow F(\psi)$. 

\textbf{Case} $\policy = \forall\vec{x}.(g\rightarrow\policy)$: 
According to the definition of \ereduce, if $\ereduce(\cL, \forall\vec{x}.(g\rightarrow\policy), \emptyset,\sigma)\Downarrow\psi$,  
then we have, 
$\sathat(\cL,g,\emptyset,\sigma)\Downarrow \Sigma'$, 
$\forall\sigma_i\in\Sigma'.\ereduce(\cL,\policy,\emptyset,\sigma_i)\Downarrow \policy_i$, and 
$\psi\leftarrow\bigwedge_i\policy_i\wedge\forall\vec{x}.(g\wedge\vec{x}\notin[\Sigma'\downarrow\vec{x}]\rightarrow\policy)$. 
From the correctness of \sathat (Lemma~\ref{lemma:correctnessSathat}), if  
$\sathat(\cL,g,\emptyset,\sigma)\Downarrow \Sigma'$, then 
$\sathat(F(\cL),F(g),\emptyset,F(\sigma))\Downarrow F(\Sigma')$. 
For all $1\leq i \leq |\Sigma|$, if $\sigma_i\in\Sigma$ and $\sigma'_i\in F(\Sigma)$, 
then $F(\sigma_i) = \sigma'_i$. From inductive hypothesis, if 
$\forall\sigma_i\in\Sigma'.\ereduce(\cL,\policy,\emptyset,\sigma_i)\Downarrow \policy_i$ 
then $\forall\sigma'_i\in F(\Sigma').\ereduce(F(\cL), F(\policy),\emptyset,\sigma'_i)\Downarrow F(\policy_i)$. 
Thus, we can show that $\ereduce(F(\cL), F(\forall\vec{x}.(g\rightarrow\policy)), \emptyset,F(\sigma))\Downarrow F(\psi)$. 

The rest of the cases are similar. 
\end{proof}

\begin{proposition}[Functional correctness of \ereduce in random oracle model]\label{proposition:correctnessReduceRO}
For any policy \policy such that there exists $\inp$ and $\mymap$ such that 
$\inp\nsat\policy:\mymap$, for any schema \cS, for any plaintext log $\cL=\langle \db, \cT\rangle$, 
for all substitution $\sigma$ such that $\pred{MappedVariables}(\sigma)\supseteq \pred{FE}(\inp)$ and $\pred{Source}(\sigma)\supseteq\inp$, for all equality scheme \escheme 
and 
the set of column equivalence classes $E=\{E_i\}_{i=1}^n$ obtained from \escheme, for all random oracle  
set $R =\{r_i\}_{i=1}^n$ where $r_i$'s domain contains all values in the equivalent class $E_i$, 
if $\ereduce(\cL,\policy,\emptyset,\sigma)\Downarrow\psi$ then 
$\ereduce(F(\cL),F(\policy),\emptyset,F(\sigma))\Downarrow F(\psi)$.  
\end{proposition}
\begin{proof}
As the random oracle is an injective function the proof follows from Lemma~\ref{lemma:correctnessReduce}. 
\end{proof}



%\noindent 
%\textbf{Generalized pseudorandom function security :}
%Generalized pseudorandom function security game is defined for a sufficiently large security parameter \param and 
%for any $n = \pred{poly}(\param)$, between a challenger \cl and an adaptive, ppt adversary \adv. The game proceeds 
%as follows: 
%\begin{enumerate}
%\item \cl probabilistically generate $n$ keys $\{K_i\}_{i=1}^n$ using the \pred{KeyGen} function. 
%$\{K_i\}_{i=1}^n\leftarrow\pred{KeyGen}(1^\param,n)$.
%\item \cl uses keys in $\{K_i\}_{i=1}^n$ to choose $n$ pseudorandom function (PRF) $F=\{PRF_{K_1},\ldots, PRF_{K_n}\}$ from the pseudorandom function family. 
%\item \cl also chooses $n$ instances of random oracle $RO = \{R_1, \ldots, R_n\}$. 
%\item \cl probabilistically chooses a bit $b$. $b\overset{\$}{\leftarrow}\{0,1\}$.  
%\item Then there is a polynomial of \param number of rounds of engagement between \cl and \adv. At each round $j$:
%\begin{enumerate}
%\item \adv adaptively chooses $n$ plaintext message $m^i = \{m^i_j\}_{j=1}^n$  and sends it to \cl. 
%\item If $b=0$, \cl returns the following transformed messages $\{M0^i_j\}_{j=1}^n = F(\{m^i_j\}_{j=1}^n)$ to \adv. 
%Else   \cl returns the following transformed messages $\{M1^i_j\}_{j=1}^n = RO(\{m^i_j\}_{j=1}^n)$. 
%\end{enumerate}
%\item \adv makes a guess $b'$ of the bit $b$. 
%\end{enumerate}  
%$\pred{win}^\adv$ represents the indicator random variable indicating whether \adv wins the above game ($\pred{win}^\adv=1$ denoted that  
%\adv wins the above game and $\pred{win}^\adv=0$ represents \adv loses the game).  
%\begin{corollary}\label{corollary:GPRFS}
%For all sufficiently large \param and for all $n = \pred{poly}(\param)$, $\pred{Pr}[\pred{win}^\adv=1]\leq\pred{negl}(\param)$ 
%where the probability is taken over the random coins 
%used by \adv as well as the random coins used in choosing the key and the random 
%bit $b$. 
%\end{corollary}
%\begin{proof}
%The proof is by standard hybrid argument. 
%%Consider the following sequence of games: 

%%Game 0: This game is exactly like the above game. 

%%$\vdots$

%%Game $j$: In this game, we just replace $PRF_{K_j}$ with a random oracle instance $RO_j$. 
%%$\pred{win}^\adv_j$ represents the indicator random variable indicating whether \adv wins 
%%in Game $j$. 

%%$\vdots$

%%Game $n$: In this game, we just replace $PRF_{K_n}$ with a random oracle instance $RO_n$. 
%%$\pred{win}^\adv_n$ represents the indicator random variable indicating whether \adv wins 
%%in Game $n$. Note that, in this game all instances of pseudorandom functions have been replaced 
%%by instances of random oracles. 

%%By hybrid argument we know for any $j > 0$, 
%%$|\pred{Pr}[\pred{win}^\adv_j = 1 ] - \pred{Pr}[\pred{win}^\adv_{(j_1)}]| \leq \pred{negl}(\param)$. 
%%As $n=\pred{poly}(\param)$ and $n\times\pred{negl}(\param) \simeq \pred{negl}(\param)$, we can write:  
%%$|\pred{Pr}[\pred{win}^\adv_0 = 1 ] - \pred{Pr}[\pred{win}^\adv_n]| \leq \pred{negl}(\param)$. 

%%It is trivial that the \adv's advantage of distinguishing two $n$ instances of random oracle is $\pred{negl}(\param)$. 
%%Hence, $\pred{Pr}[\pred{win}^\adv_n] = \pred{negl}(\param)$. From which we can write 
%%$\pred{Pr}[\pred{win}^\adv_0 = 1 ] = \pred{negl}(\param) + \pred{negl}(\param) \simeq \pred{negl}(\param)$. 
%\end{proof}


%Now from Proposition~\ref{proposition:correctnessReduceRO} and Corollary~\ref{corollary:GPRFS}, we have the 
%correctness of \ereduce in \dt. 

\begin{theorem}[Correctness of \ereduce in \dt]
Assuming deterministic encryption is a pseudorandom permutation, 
for any policy \policy such that there exists $\inp$ and $\mymap$ so that 
$\inp\nsat\policy:\mymap$, for any schema \cS, for any plaintext log $\cL=\langle \db, \cT\rangle$, 
for all substitution $\sigma$ such that $\pred{MappedVariables}(\sigma)\supseteq \pred{FE}(\inp)$ and $\pred{Source}(\sigma)\supseteq\inp$, for all equality scheme \escheme 
and 
the set of column equivalence classes $E=\{E_i\}_{i=1}^n$ obtained from \escheme, for all injective function 
set $F =\{\deter(\cdot, k_i)\}_{i=1}^n$ where 
$\deter(\cdot, k_i)$ is the deterministic encryption function with same randomly generated key $k_i$ where 
the domain of the \deter function comprises of all values in the equivalent class $E_i$, 
if $\ereduce(\cL,\policy,\emptyset,\sigma)\Downarrow\psi$ then 
$\ereduce(F(\cL),F(\policy),\emptyset,F(\sigma))\Downarrow F(\psi)$.  
\end{theorem}
\begin{proof}
The proof is by contradiction. 
Let us assume that \ereduce is incorrect with non-negligible probability 
when the injective functions are replaced by deterministic encryption. 
That is  given $\ereduce(\cL,\policy,\emptyset,\sigma)\Downarrow\psi$ and 
$F =\{\deter(\cdot, k_i)\}_{i=1}^n$, $\ereduce(F(\cL),F(\policy),\emptyset,F(\sigma))\Downarrow F(\psi')$ where 
$\psi' \neq \psi$. 
As deterministic encryption can be considered a pseudorandom permutation (consequently a pseudorandom function), if  \ereduce 
is incorrect with non-negligible probability, additionally as the adversary has access to the plaintext log \cL 
and the result of \ereduce over \cL, comparing the result of \ereduce in the random oracle case and the deterministic encryption case, 
it can differentiate random oracle from a pseudorandom function with non-negligible property, which is a contradiction. 
This completes our proof. 
\end{proof}

%As deterministic encryption is a pseudorandom permutation (consequently pseudorandom function), 
%it follows from Proposition~\ref{proposition:correctnessReduceRO} and Corollary~\ref{corollary:GPRFS} 
%\ereduce is correct in \dt. This is easy to understand intuitively. If \ereduce were not to be correct 
%in \dt with non-negligible probability, then adversary could use the residual formula returned by \ereduce to differentiate 
%a pseudorandom function and random oracle with non-negligible probability. 



==> correctness2.tex <==
%\begin{lemma}\label{lemma:correctness}
%For all plaintext policies $\policy_\pred{P}$ and $\psi_\pred{P}$, for all encrypted policies $\policy_\pred{E}$ and $\psi_\pred{E}$, 
%for all database schema  \cS, 
%for all plaintext audit logs $\cL=\langle\db, \cT\rangle$, 
%for all encrypted audit logs $e\cL=\langle e\db, e\cT\rangle$, 
%for all plaintext substitution $\sigma_\pred{P}$, 
%for all encrypted substitution $\sigma_\pred{E}$, 
%for all \inp, 
%for all equality scheme \escheme, 
%for all security parameter \param,  
%for all encryption keys \keys, 
%for all token list $\vec{\Delta}$
%such that: 
%\begin{itemize}\setlength{\itemsep}{0em}
%\item $\inp\nsat\policy_\pred{P}: \mymap$, 
%\item $\sigma_\pred{P}$ is \emph{consistent} with \inp, 
%\item $\keys = \pred{KeyGen}^\pred{KH}(\param,\cS)$, 
%\item $\psi_\pred{P} = \reduce(\cL,\sigma_\pred{P},\policy_\pred{P})$, 
%\item $\vec{\Delta} = \pred{GenerateToken}(\cS,\escheme, \keys)$, 
%\item $e\cL = \pred{EncryptLog}^{\pred{KH}}(\cL, \cS, \keys)$, 
%\item $\policy_\pred{E} = \pred{EncryptPolicyConstants}^{\pred{KH}}(\policy_\pred{P},\keys)$, 
%\item $\sigma_\pred{E} = \pred{EncryptSubstitution}^{\pred{KH}}(\sigma_\pred{P},\keys)$, 
%\item \pred{AKH} key adjustment algorithm is correct, 
%\item $\psi_\pred{E} = \ereduce^{\pred{KH}}(e\cL,\policy_\pred{E},\vec{\Delta},\sigma_\pred{E})$, and 
%\item $\psi'_\pred{P} = \pred{DecryptPolicyConstants}^{\pred{KH}}(\psi_\pred{E},\keys)$,   
%\end{itemize} 
%if $\psi_\pred{p} \neq \psi'_\pred{P}$ then there is a hash collision. 
%\end{lemma}
%\begin{proof}
%By structural induction on $\policy_\pred{P}$. 
%\end{proof} 

We have proved that \ereduce is correct for audit logs encrypted with both \dt and \kh. 
The correctness theorem for $\ereduce^{\pred{DET}}$ (not shown due to space limitation) 
states that, for any plaintext log \cL whose \dt encrypted counterpart is $e\cL$ and 
any well-moded policy $\policy_\pred{P}$ whose \dt encrypted counterpart is $\policy_\pred{E}$, 
if we run \reduce with respect to \cL and $\policy_\pred{P}$ to get the residual formula $\psi_\pred{P}$ 
and run \ereduce with respect to $e\cL$ and $\policy_\pred{E}$ to get the residual formula $\psi_\pred{E}$, 
then if we decrypt $\psi_\pred{E}$ it be equal to $\psi_\pred{P}$. However, in case of \kh, our correctness 
theorem (Theorem~\ref{thm:khcorrectness}) states that the decrypted result of \ereduce and the result of \reduce 
are equal with high probability. The results may not be equal due to hash collisions. 
%We prove Theorem~\ref{thm:khcorrectness} 
%by first proving a lemma stating that if the residuals are not equal then there must be hash collision(s). 
Due to space requirement 
we do not show the proofs here. 

%\begin{theorem}[Correctness of $\ereduce^{\pred{DET}}$]
%For all plaintext policies $\policy_\pred{P}$ and $\psi_\pred{P}$, for all constant 
%encrypted policies $\policy_\pred{E}$ and $\psi_\pred{E}$, 
%for all database schema  \cS, 
%for all plaintext audit logs $\cL=\langle\db, \cT\rangle$, 
%for all encrypted audit logs $e\cL=\langle e\db, e\cT\rangle$, 
%for all plaintext substitution $\sigma_\pred{P}$, 
%for all encrypted substitution $\sigma_\pred{E}$, 
%for all \inp, 
%for all equality scheme \escheme, 
%for all security parameter \param,
%for all encryption keys \keys if all of the following hold:  
%(1) $\inp\nsat\policy_\pred{P}: \mymap$, 
%(2) $\sigma_\pred{P}$ is \emph{consistent} with \inp, 
%(3) $\keys = \pred{KeyGen}^\pred{KH}(1^\param,\cS,\mymap)$, 
%(4) $e\cL = \pred{EncryptLog}^{\pred{DET}}(\cL, \cS, \keys)$, 
%(5) $\policy_\pred{E} = \pred{EncryptPolicyConstants}^{\pred{DET}}(\policy_\pred{P},\keys)$, 
%(6) $\sigma_\pred{E} = \pred{EncryptSu}\\\pred{bstitution}^{\pred{DET}}(\sigma_\pred{P},\keys)$, 
%(7) $\psi_\pred{P} = \reduce(\cL,\sigma_\pred{P},\policy_\pred{P})$, 
%(8) $\psi_\pred{E} = \ereduce^{\pred{DET}}(e\cL,\policy_\pred{E},\sigma_\pred{E})$, and 
%(9) $\psi'_\pred{P} = \pred{DecryptPolicyConstan}\\\pred{ts}^{\pred{DET}}(\psi_\pred{E},\keys)$,   
%then $\psi_\pred{p} = \psi'_\pred{P}$. 
%\end{theorem} 
%\begin{proof}
%Proof by induction on the structure of $\policy_\pred{P}$. 
%\end{proof} 


\begin{theorem}[Correctness of $\ereduce^{\pred{KH}}$]\label{thm:khcorrectness}
For all plaintext policies $\policy_\pred{P}$ and $\psi_\pred{P}$, 
for all constant encrypted policies $\policy_\pred{E}$ and $\psi_\pred{E}$, 
for all database schema  \cS, 
for all plaintext audit logs $\cL=\langle\db, \cT\rangle$, 
for all encrypted audit logs $e\cL=\langle e\db, e\cT\rangle$, 
for all plaintext substitution $\sigma_\pred{P}$, 
for all encrypted substitution $\sigma_\pred{E}$, 
for all \inp, 
for all equality scheme \escheme, 
for all security parameter \param,
for all encryption keys \keys, 
for all token list $\vec{\Delta}$, if all of the following holds:   
(1) $\inp\nsat\policy_\pred{P}: \mymap$, 
(2) $[\sigma_\pred{P}]\supseteq\inp$, 
(3) $\keys = \pred{KeyGen}^\pred{KH}(\param,\cS)$, $\vec{\Delta} = \pred{GenerateToken}(\cS,\escheme, \keys)$, 
(4) $e\cL = \pred{EncryptLog}^{\pred{KH}}(\cL, \cS, \keys)$, 
(5) $\policy_\pred{E} = \pred{EncryptPolicyConstants}^{\pred{KH}}(\policy_\pred{P}\\,\keys)$, 
(6) \pred{AKH} key adjustment  is correct, 
(7) $\sigma_\pred{E} = \pred{EncryptSub}\\\pred{stitution}^{\pred{KH}}(\sigma_\pred{P},\keys)$, 
(8) $\psi_\pred{P} = \reduce(\cL,\sigma_\pred{P},\policy_\pred{P})$, 
(9) $\psi_\pred{E} = \ereduce^{\pred{KH}}(e\cL,\policy_\pred{E},\vec{\Delta},\sigma_\pred{E})$, and 
(10) $\psi'_\pred{P} = \pred{DecryptPolicyConst}\\\pred{ants}^{\pred{KH}}(\psi_\pred{E},\keys)$,   
then $\psi_\pred{p} = \psi'_\pred{P}$ with high probability. 
\end{theorem} 
\begin{proof}
We first prove that if $\psi_\pred{p} \neq \psi'_\pred{P}$ then there is hash collision(s). As the probability of 
hash collision is negligible, we  conclude that $\psi_\pred{p} = \psi'_\pred{P}$ with high probability. 
\end{proof} 


==> security.tex <==
In this section, we will first present the security analysis of the \DOPE data-structure then 
we will present the end-to-end security analysis of \detkh. 

\subsection{Security definition of \DOPE scheme}
We now present the security definition of our \DOPE scheme in \dt instance (definition for \kh instance is similar) where
the definition asserts that the scheme leaks the order
between \emph{all} ciphertexts in the \DOPE data-structure 
and  distances between \emph{some}
of the ciphertexts in the system. We call the security definition of \DOPE, \DOCPA (\emph{indistinguishability
under distance-ordered chosen plaintext attack}) which we adopt from the \OCPA (\emph{indistinguishability
under ordered chosen plaintext attack}) definition by Boldyreva~\etal~\cite{BCLO} and \LOR security definition 
by Pandey and Rouselakis~\cite{PR12}.
%A scheme is \OCPA if the only information
%it leaks is the order between all the ciphertexts whereas a scheme is \DOCPA if it leaks the order between
%all ciphertexts in the \DOPE data-structure and additionally leaks some predefined  distances between some of ciphertexts.
Given a set of predefined distances $D =\{d_1,  \ldots, d_n\}$ such that $0\in D$ and $D\subset\mathbb{N}$, 
we say two sequences $\vec{u}=[u_1, \ldots, u_m]$
and $\vec{v}=[v_1, \ldots, v_m]$ have the \emph{distance-ordered equality pattern}
with respect to $D$, denoted by $\pred{DOEP}(\vec{u},\vec{v},D)$,
if and only if  the following holds:
$\forall i, j, k, l. (1\leq i, j \leq m \wedge 1 \leq k, l\leq n\Longrightarrow\left(
u_i + d_k \geq u_j + d_l \Longleftrightarrow v_i + d_k \geq v_j + d_l\right))$.
Finally, a scheme having \DOCPA security ensures that the adversary cannot distinguish
between encryptions of two different sequences (\eg, $\vec{u}$ and $\vec{v}$) if they have the distance-ordered equality
pattern for a given $D$.

\noindent 
\textbf{\DOCPA security game:}
The \DOCPA security game between a client \cl (\ie, owner of the
encrypted audit log) and an adaptive, probabilistic polynomial time (in short, ppt) adversary \adv (\ie, the cloud service provider)
for the security parameter \param proceeds as follows:
\begin{enumerate}
 \item \cl generates a secret key \sk using the probabilistic key generation algorithm \keygen.
$\sk\overset{\$}{\leftarrow} \keygen(1^\param)$.

 \item \cl chooses a random bit $b$.
$b\overset{\$}{\leftarrow}\{0, 1\}$.
  \item \cl chooses a set of  distances $D =\{d_1,\ldots,d_n\}$. %such that $D\subset\mathbb{N}$ and $0\in D$.
  \item \cl sends the set $D$ to \adv.
 \item \cl and \adv engages in a polynomial of \param number of rounds of interactions.
 In each round $j$:
 \begin{enumerate}
  \item \adv selects two values $v^0_j$ and $v^1_j$ and sends them to \cl.
  \item While \adv is observing, \cl interacts with the \DOPE data-structure to deterministically encrypt the following $n+1$ values %using 
$v^b_j$, $v^b_j + d_1, v^b_j + d_2, \ldots, v^b_j + d_n$ using
%  the deterministic encrypt function \deter with the secret key 
\sk. 
% while the adversary \adv observing all the interactions and state of \server.
  \item While \adv is observing, \cl again interacts \DOPE data-structure to establish the association
  between two ciphertexts  $\deter(v^b_j, \sk)$ and $\deter(v^b_j+d_i, \sk)$ and a distance $d_i$,
  that is
  $\deter(v^b_j, \sk)\overset{d_i}{\Longrightarrow}\deter(v^b_j+d_i, \sk)$
  for all $i$ such that $1\leq i\leq n$. 
%The adversary \adv observes all the interactions
%  between \cl and \server and all the states in \server in this step.
 \end{enumerate}
 \item \adv then outputs his guess of $b$, $b'$. 
%which is a guess for the bit $b$.
\end{enumerate}

%\noindent
%\textbf{Winning condition}:
%The adversary 
\adv wins the \DOCPA security game if and only if: 
%the following holds:
\begin{enumerate}
\item \adv guesses  $b$ correctly (\ie, $b=b'$);
\item 
%The sequences $\{v^0_j\}_m$ and $\{v^1_j\}_m$ have the same
%distance-ordered equality pattern for the given $D$, \ie, 
$\pred{DOEP}(\{v^0_j\}_m,\{v^1_j\}_m,D)$ holds. 
\item $\{v^0_j\}_m \neq \{v^1_j\}_m$. 
\end{enumerate}
% We consider $\mathsf{win}^{\adv, k}$ to be an indicator random variable which
% indicates the \adv's success of winning the above \DOCPA security game.

\begin{definition}[\DOCPA]
A \DOPE scheme is \DOCPA secure 
if for all ppt adversary \adv and for all sufficiently large value 
%of the security
%parameter 
\param,
if the following holds:
% \noindent
$\mathsf{Pr}[\mathsf{win}^{\adv, k}]\leq \frac{1}{2} + \mathsf{neg}(\param)$. 
%where
\end{definition}
$\mathsf{win}^{\adv, k}$ is an indicator random variable which
indicates the \adv's success of winning the above \DOCPA security game.
A function $f:\mathbb{N}\rightarrow\mathbb{R}$ is \emph{negligible} with respect to its
argument \param, if for every  $c\in\mathbb{N}$ there exists another integer $K$ such that
for all $\param > K$, $f(\param) < x^{-c}$. For ease of exposition,
we write $f(\param) = \pred{negl}(\param)$ for all sufficiently large $\param$.

\begin{theorem}\label{theorem:dopeSecurity}%[\DOPE Security\label{theorem:dopeSecurity}]
Our \DOPE scheme is \DOCPA secure. 
%according to the \DOCPA security definition.
\end{theorem}

\begin{proof}
The proof is straightforward using the hybrid argument. It can be carried out
by slightly enhancing the security proof of \MOPE scheme, having the
\OCPA security~\cite{mope}, to consider the \pred{DOEP}  restriction.
\end{proof}


\subsection{Overall System Security Definition}
In this section, we present the overall security
analysis of 
%definition of our auditing over encrypted log framework 
\dt and the security analysis for \kh follows from it. For the following discussion, we will 
consider the \dt instance unless 
specified otherwise. 
We provide an indistinguishability kind of security definition for
the overall security guarantee of our framework \dt.
We call the security definition \ECPLA, which is short for, \emph{indistinguishability
under equivalent chosen plaintext log attack}.
Intuitively, the security definition states that
given two \emph{equivalent}
plaintext audit logs (see Definition~\ref{def:plainLogEquivalence}), if we encrypt
one of the audit logs and make the result and the execution of
\ereduce 
%running the compliance checking algorithm 
over the encrypted audit log
available to the adversary then the adversary cannot distinguish
which plaintext audit log was encrypted. More specifically, if the
adversary observes the result and the execution of \ereduce 
%the compliance checking
%algorithm 
over an encrypted audit log, it cannot with high probability distinguish 
the encrypted audit log in question and any other audit logs in the same 
equivalent class.
For a given encrypted audit log it leaks the
equivalent class in which the log is a member.
%We later show how to  construct
%a dummy audit log $\cL_d$ given any plaintext log $\cL$
%such that $\cL$ and $\cL_d$ are equivalent.


\subsubsection{Equivalent Plaintext Audit Logs}
We now  define what it means for two plaintext logs to be
equivalent with respect to a set of constants $C$ and a set of
time distances $D$. We call a distance set $D$ \emph{well-formed}
with respect to $C$
if and only if $D\subseteq C$, $D\subset \mathbb{N}$, and $0\in D$.
Note that, we write $D$ is a well-formed set of distances when the
$C$ is understood from the context.
\begin{definition}[Plaintext log equivalence]\label{def:plainLogEquivalence}
Given two plaintext audit logs $\cL_1$ and $\cL_2$,
a set of constants $C$ and a well-formed set of distances $D$,
$\cL_1$ and $\cL_2$ are equivalent, denoted by $\cL_1\equiv_{(C,D)}\cL_2$, if and only if all of the
followings hold:
\begin{enumerate}
\item Both the plaintext audit logs $\cL_1$ and $\cL_2$ are well-formed.
\item Both the plaintext audit logs have the same schema.
\item The sequence of unique time stamps appearing in $\cL_1$ and
$\cL_2$, respectively, satisfy the distance-ordered equality pattern with respect to $D$,
\ie,
$\pred{DOEP}(\pred{timeStamps}(\cL_1), \pred{timeStamps}(\cL_2), D)$ holds. The function
$\pred{timeStamps}(\cdot)$ takes as input an audit log  and returns
all the unique time stamps in that audit log in the insertion order. 
\item There exists a bijection $\mathcal{M}_p$
from the domain of $\cL_1$  to the domain of $\cL_2$,
$\mathcal{M}_p: \cD(\cL_1)\rightarrow\cD(\cL_2)$, such that:
\begin{enumerate}
    \item Each constant in set $C$, either appears in both $\cL_1$ and $\cL_2$ or 
appears in none. 
%the domain of both the plaintext
%    audit logs or does not appear in the domain of either of the plaintext audit logs.
    That is, $\forall c\in C. c\in\cD(\cL_1)\leftrightarrow c\in\cD(\cL_2)$ holds.
\item Each constant in set $C$, if it appears 
%in the domain of both the plaintext
%audit logs 
$\cL_1$ and $\cL_2$ 
then according to $\cM_p$ they are mapped to itself.
That is  $\forall c\in C.c\in\cD(\cL_1)\wedge c\in\cD(\cL_2)\rightarrow \cM_p(c) = c$.
\item Each element $x$ in $\cL_1$'s domain 
is mapped to another element $y$ in $\cL_2$'s domain such that $|x|=|y|$. 
That is $\forall x\in\cD(\cL_1). |x| = |\cM(x)|$. 

\item Both $\cL_1$ and $\cL_2$ respect the mapping $\mathcal{M}_p$. That is
for any table \pred{tbl} in both $\cL_1$ and $\cL_2$,
there is a bijection $\cM_r$ from the rows in \pred{tbl} of $\cL_1$
to the rows in \pred{tbl} of $\cL_2$, such that if we take any row $r_1$
of $\pred{tbl}$ in $\cL_1$ such that $\cM_r(r_1) = r_2$ where $r_2$ is a
row of \pred{tbl} in $\cL_2$ then replacing all elements of $r_1$ according
to $\cM_p$ will result in the row $r_2$.

\end{enumerate}
\end{enumerate}
\end{definition}

\subsubsection{Equivalent Encrypted Audit Logs}
We now define 
%what it means for two 
encrypted audit log equivalence. The definition 
of equivalence was chosen carefully such that we have Corollary~\ref{corollary:peLogEquivalence} which 
states that if we encrypt two equivalent plaintext audit logs 
based on the same keying scheme \kscheme and key set \keys then the resulting encrypted audit logs will be equivalent 
according to the definition below.  
\begin{definition}[Encrypted audit log equivalence]\label{def:encryptedLogEquivalence}
For any two encrypted audit logs $e\cL_1=\langle e\dbd{1}, e\cT_1\rangle$ and $e\cL_2=\langle e\dbd{2}, e\cT_2\rangle$, 
any set of constants $C$, any set of well-formed distances $D$, for any keying scheme \kscheme, for any key set \keys 
such that \keys is consistent with \kscheme, we say $e\cL_1$ is \emph{equivalent} to $e\cL_2$, denoted by 
$e\cL_1\equiv_{(C,D,\kscheme,\keys)}e\cL_2$, if and only if all of the followings hold: 
\begin{enumerate}
\item $e\dbd{1}$ and $e\dbd{2}$ are both well-formed. 
\item $e\dbd{1}$ and $e\dbd{2}$ have the same schema. 
\item $\forall i\in\{1,2\},\forall et\in \ets(e\dbd{i}). et\in e\cT_i$. The function
$\ets(\cdot)$ takes as input a database representation of an encrypted audit log  and returns
all the unique encrypted time stamps in that audit log in the insertion order.  
\item $\forall i\in\{1,2\},\forall et\in \ets(e\dbd{i}),\forall (1\leq j\leq|D|), \exists pt, k. k\in\keys \wedge et = \deter(pt,k)\wedge \deter(pt+d_j,k)\in e\cT_i$. 
The $\deter(\cdot, \cdot)$ function 
takes as input a plaintext value $pt$ and an encryption key $k$, and deterministically encrypt $pt$ with $k$ and returns the ciphertext. 
\item There exists a bijection $\mathcal{M}_e$
from the domain of $e\cL_1$ to the domain of $e\cL_2$, 
$\mathcal{M}_e: e\cD(e\cL_1)\rightarrow e\cD(e\cL_2)$, such that:
\begin{enumerate}
    \item Each constant in set $C$, either appears in both $e\cL_1$ and $e\cL_2$ or appears in none. 
%in the domain of both the encrypted 
%    audit logs or does not appear in the domain of either of the encrypted audit logs.
    That is, $\forall c\in C, \forall k\in\keys. \deter(c, k)\in e\cD(e\cL_1) \leftrightarrow \deter(c, k)\in e\cD(e\cL_2)$ holds.  

\item Each constant in set $C$, if it appears in both $e\cL_1$ and $e\cL_2$ then according to $\cM_e$ they are mapped to itself.
Hence the following holds:  
$\forall c\in C, \forall k\in\keys. \deter(c, k)\in e\cD(e\cL_1) \wedge \deter(c, k)\in e\cD(e\cL_2)\rightarrow\cM_e(\deter(c,k)) = \deter(c,k)$.


\item $e\cL_1$ and $e\cL_2$ respect the mapping $\mathcal{M}_e$. That is
for any table \pred{tbl} that appears in both $e\cL_1$ and $e\cL_2$,
there is a bijection $e\cM_r$ from the rows in \pred{tbl} of $e\cL_1$
to the rows in \pred{tbl} of $e\cL_2$, such that if we take any row $r_1$
of $\pred{tbl}$ in $e\cL_1$ such that $e\cM_r(r_1) = r_2$ where $r_2$ is a
row of \pred{tbl} in $e\cL_2$ then replacing all elements of $r_1$ according
to $\cM_e$ will result in the row $r_2$.

\item If we take the  \DOPE data-structure $e\cT_1$ and replace all concrete encrypted values 
according to the mapping $\cM_e$, then we will get the second  \DOPE data-structure $e\cT_2$ and 
vice versa. 
\end{enumerate}
\end{enumerate}
\end{definition} 

\begin{corollary}\label{corollary:peLogEquivalence}
For any two plaintext audit logs $\cL_1$ and $\cL_2$ with the same database schema \cS, for any set of constants $C$, for any set of well formed distances $D$, 
for any keying scheme \kscheme, for any key sets \keys, such that \keys is consistent with \kscheme, if $\cL_1\equiv_{(C,D)}\cL_2$ 
then $e\cL_1\equiv_{(C,D,\kscheme,\keys)}e\cL_2$ where $e\cL_i=\langle e\dbd{i}, e\cT_i\rangle\leftarrow \pred{EncryptLog}^\pred{DET}(\cL_i, \cS, \keys)$ where $i\in\{1,2\}$. 
\end{corollary}


\subsubsection{\SQECPLA security definition}
Before we prove that \dt is \ECPLA secure we first introduce
the readers with another security definition, \SQECPLA (short for,
\emph{indistinguishability under selective query chosen plaintext
log attack}), which we will use to prove \detkh's overall security
guarantee.
The \SQECPLA game is played  between a challenger \cl (the client or
the owner of the plaintext audit log) and an adaptive, ppt adversary \adv
(the cloud service provider in our setting). Although, in our normal setting we assume the
\adv to be honest but curious, in the current security definition we give \adv 
ability to selectively query the encrypted audit log.
The \SQECPLA security intuitively requires that for a given
set of constants $C$ and a well-formed set of distances $D$, if we allow \adv access to
results for select queries (the same set of queries \ereduce makes to the log) 
over an encrypted audit log $e\cL=\langle e\db, e\cT\rangle$
which is the encryption of one of the \adv chosen plaintext audit logs $\cL_0$ or $\cL_1$
 such that $\cL_0\equiv_{(C,D)}\cL_1$, then \adv
cannot assert with high probability which plaintext audit log's encryption
 he observed. 

\paragraph*{\textbf{\SQECPLA security game}}
The \SQECPLA game is played for all large enough security parameter \param, 
for any constant set $C$, for any well-formed distance set $D$, 
for any database schema \cS, 
for all predicate  set $\mathbb{P}$, 
for any coherent keying scheme \kscheme, and it proceeds as follows. 
In the current context, we consider that $\mathbb{P}$ contains all table names in \cS and we 
use this to be consistent with the signature of $\pred{KeyGen}^\pred{DET}$. 
\begin{enumerate}
\item \cl probabilistically generates a set of secret keys \keys based on the sufficiently large security parameter \param, 
the database schema \cS, and the 
keying scheme \kscheme. 
$\keys\overset{\$}{\leftarrow} \pred{KeyGen}^\pred{DET}(1^\param, \mathbb{P}, \cS, \kscheme)$.
\item \cl randomly  selects a bit $b$. 
$b\overset{\$}{\leftarrow}\{0,1\}$.
\item \cl sends \cS, $C$, $D$, the encryption of $C$ with key corresponding to columns in which $C$ appears, and 
the encryption of $D$ with key $K_\pred{time}$  to  \adv.  
\item \adv adaptively chooses two plaintext audit logs $\cL_0$ and $\cL_1$ such that both $\cL_0, \cL_1$ have  schema  
schema \cS, $\cL_0\equiv_{(C,D)}\cL_1$, $\cL_0\neq \cL_1$, and sends $\cL_0$, $\cL_1$
to  \cl.

\item \cl deterministically encrypts $\cL_b$ to obtain the encrypted audit log $\langle e\dbd{b}, e\cT_b\rangle$ 
according to the data schema \cS  and key set \keys. \adv observes the construction of 
the \DOPE data-structure $e\cT_b$. 
$\langle e\dbd{b}, e\cT_b\rangle\leftarrow\pred{EncryptLog}^\pred{DET}(\cL_b, \cS, \keys)$. 


\item Then there are a polynomial of \param number of rounds played between \cl and \adv. In each round $i$,
\adv asks one of the following types of query $q$. \cl runs the query $q$ on 
$\langle e\dbd{b}, e\cT_b\rangle$ and returns the result to \adv.
\begin{description}%[{(\pred{Q}-a)}]
\item[\textbf{Selection query:}] \hfill\\ 
Select all tuples from a table \pred{tbl} of the encrypted audit log $\langle e\dbd{b}, e\cT_b\rangle$.
\item[\textbf{Constrained selection query:}] \hfill \\
Select all tuples from a table \pred{tbl} of the encrypted audit log $\langle e\dbd{b}, e\cT_b\rangle$ where $\bigwedge_i (x_i=ec_i)$, in which $x_i$ is a
column name of table \pred{tbl} and $ec_i$ is a ciphertext drawn from the domain of $\langle e\dbd{b}, e\cT_b\rangle$.
\item[\textbf{Time-Order query:}] \hfill\\ 
For all $d_1,d_2\in D$, for all encrypted time stamps $et_1,et_2$ in $e\dbd{b}$, 

$e\cT_b.\pred{timeOrder}(et_1,d_1,et_2,d_2) \overset{?}{=}\top$.
\end{description}
\item \adv then outputs his guess bit $b'$ of $b$.
\end{enumerate}

\adv wins the above \SQECPLA game if and
only if $b=b'$ and \adv does not ask for the encryption of a non-constant value in either 
of the domain. 
Let us denote the random variable indicating the success of \adv winning the above \ECPLA game by
$\pred{win}^{\adv, \param, C,D}_{\pred{SQ}}$.

\begin{definition}[\SQECPLA: Indistinguishability under selective query chosen plaintext
log attack]
Any encrypted auditing framework is \SQECPLA secure if and only if for all ppt \adv, 
all constant sets $C$ and all well-formed distance set $D$, for all database schema \cS, 
for all predicate set $\mathbb{P}$, 
for all coherent keying scheme \kscheme, and for all sufficiently large security parameter $\param$,
$\pred{Pr}[\pred{win}^{\adv, \param,C,D}_{\pred{SQ}}]\leq \frac{1}{2} + \pred{negl}(\param)$.
\end{definition}
Finally, we have the following lemma which states that \dt  
is \SQECPLA secure.  
\begin{lemma}\label{lemma:SQECPLA}
\dt is \SQECPLA secure.
\end{lemma}

\begin{proof}
Let us consider the \adv in the \SQECPLA game to be any ppt adversary.  
Let us also consider $\{k_i\}^n_{i=1} = \{K \mid \exists t, c. \langle t, c, K\rangle\in\keys\}$. 
We also consider that the random oracle $\pred{RO}$ returns a random value $v_r$ the first time it
sees an input value $v$. If $\pred{RO}$ is called again with the same input value $v$, then it returns the
same random value $v_r$. We will prove the lemma using a sequence of $n+1$ games and using the standard hybrid argument.

\textbf{Game 0}: This game is exactly like the \SQECPLA game. Let us consider that 
$\pred{H}^0(\param)$ denotes the indicator random variable
which indicates whether the \adv wins game 0.

\textbf{Game 1}: This game is almost like game 0 except we replace 
each instance of the deterministic encryption function $\deter(\cdot, k_1)$ with a 
random oracle instance $RO_1$. 
$\pred{H}^1(\param)$ denotes the indicator random variable
which indicates whether the \adv wins game 1. 



$\vdots$

\textbf{Game $n$}: This game is almost like game $n-1$ except we replace 
each instance of the deterministic encryption function $\deter(\cdot, k_n)$ with a 
random oracle instance $RO_n$. 
$\pred{H}^n(\param)$ denotes the indicator random variable
which indicates whether the \adv wins game $n$. Note that in this game all instances 
of deterministic encryption function has been replaced with instances of random oracle. 


From the definition of \emph{computationally indistinguishability}, we know that
two ensembles $\{X_\param\}_{\param\in\mathbb{N}}$
and $\{Y_\param\}_{\param\in\mathbb{N}}$ are computationally indistinguishable to any p.p.t adversary
\adv, denoted by $\{X_\param\}_{\param\in\mathbb{N}}\overset{c}{\approx}\{Y_\param\}_{\param\in\mathbb{N}}$,
if:
\begin{equation*}
\mid\pred{Pr}[\adv(X_\param, 1^\param) = 1] - \pred{Pr}[\adv(Y_\param, 1^\param)=1]\mid=\pred{negl}(\param).
\end{equation*}
As deterministic encryption function instance $\deter(\cdot, k_1)$ is a pseudorandom permutation, the following two
ensembles are \emph{computationally indistinguishable}: $\{\pred{H}^0(\param)\}_{\param\in\mathbb{N}}$
and $\{\pred{H}^1(\param)\}_{\param\in\mathbb{N}}$. From which we get:
\begin{equation*}
|\pred{Pr}[\adv(\pred{H}^0(\param), 1^\param) = 1] - \pred{Pr}[\adv(\pred{H}^1(\param), 1^\param)=1]|=\pred{negl}(\param).
\end{equation*}

As $n < \pred{poly}(\param)$  
and $n\in\mathbb{N}$, we can write $n\times \pred{negl}(\param)$ as $\pred{negl}(\param)$. From standard 
hybrid argument, we can say the following. \pred{poly}($\cdot$) represents a polynomial  function of its input argument. 
\begin{equation*}
|\pred{Pr}[\adv(\pred{H}^0(\param), 1^\param) = 1] - \pred{Pr}[\adv(\pred{H}^n(\param), 1^\param)=1]|=\pred{negl}(\param).
\end{equation*}

Now we will prove that the advantage of \adv in the game $n$ is exactly $\frac{1}{2}$. From which we can conclude
that \adv's advantage in the \SQECPLA game is maximum $\frac{1}{2} + \pred{negl}(\param)$.

By the result associated with the hybrid game 2 of Theorem~\ref{theorem:dopeSecurity}
we know \adv's advantage of differentiating $\cL_0$ and $\cL_1$
by observing the construction (\ie, insertion of elements) of $e\cT_b$ is exactly $\frac{1}{2}$.
Hence, we can conclude that just by observing the construction of  $e\cT_b$, \adv's 
advantage is exactly $\frac{1}{2}$ in the game $n$.

We will now show that \adv's advantage in game $n$ by observing the different query results
is maximum $\frac{1}{2}$. 

We will now do an induction on the rounds of the game. 
Let us consider that the advantage of \adv on game $n$ remains $\frac{1}{2}$ till the 
$(i-1)$th  round. We will show that it also remain $\frac{1}{2}$ in the $i$th round. 
Let us consider the $i$th query  and it could be one of the following form:

\noindent
\textbf{Case}-\textbf{Selection query}:
By Corollary~\ref{corollary:peLogEquivalence}, we know that 
$\langle e\dbd{0}, e\cT_0\rangle\equiv_{(C,D,\kscheme,\keys)}\langle e\dbd{1}, e\cT_1\rangle$. 
By requirement 5(c) of Definition~\ref{def:encryptedLogEquivalence}, 
if the \adv obtains all tuples from any table \pred{tbl} of the encrypted audit log $\langle e\dbd{0}, e\cT_0\rangle$
to get the rows $R_0 = r^0_1,\ldots,r^0_n$ and we apply the mapping to each rows of $R_0$ 
to obtain $R'_{1} = \cM_e(r^0_1),\ldots,\cM_e(r^0_n)$ which will be a permutation of the result we would have 
obtained if we ran the same query on the log $\langle e\dbd{1}, e\cT_1\rangle$ as the database server returns  
any results in a pseudorandom order. 
Thus, information-theoretically the adversary cannot distinguish the two audit logs 
by observing the query results. 


Additionally, as the individual values are replaced by the output of a 
random oracle, the adversary cannot guess which log each value comes from. 
This can be easily shown by designing the following experiment. 
The challenger chooses a random bit $b_1$. Then the adversary and challenger 
engages in the polynomial number of round of games. 
At each round the adversary chooses two plaintext $(m_0, m_1)$ where $m_0$ and $m_1$ are drawn from the 
domain of the audit log $\cL_0$ and $\cL_1$, respectively,  $|m_0|=|m_1|$, and $\cM(m_0) = m_1$ in which 
\cM is the bijection obtained from Definition~\ref{def:plainLogEquivalence}. 
The challenger then gives the output of a random oracle with input $m_b$ to the adversary. 
Finally, the adversary outputs a guess of the bit $b_1$. It can be easily shown that 
the adversary's advantage in this game is exactly $\frac{1}{2}$ which follows from the 
guarantee of a random oracle. 
Hence, as the adversary cannot differentiate the logs on the query results and the values 
in the query result, the adversary advantage remains $\frac{1}{2}$ even in the $i$th round.  


\noindent
\textbf{Case}-\textbf{Constrained selection query}:

Similar to the previous case.

\noindent
\textbf{Case}-\textbf{Time-Order query}:
By Corollary~\ref{corollary:peLogEquivalence} and requirements 5(c) \& 5(d) of Definition~\ref{def:encryptedLogEquivalence}, 
for any two time stamps $et_1$ and $et_2$ in $e\dbd{0}$
and for any distances $d_1, d_2\in D$, there exists $et'_1$ and $et'_2$ in $e\dbd{1}$ 
such that $\cM_e(et_1) = et'_1$ and $\cM_e(et_2) = et'_2$. 
Now by the result of the hybrid game 2 of Theorem~\ref{theorem:dopeSecurity}, 
for all $d_1, d_2\in D$,   
$\cT_0.\pred{timeOrder}(et_1, ed_1, et_2, ed_2) = \cT_1.\pred{timeOrder}(et'_1, ed_1, et'_2, ed_2)$ holds where $ed_1$ and $ed_2$ are deterministic 
encryption of $d_1$ and $d_2$, respectively, with key $K_\pred{time}$.
Hence, \adv's advantage  in game $n$ by observing the result of this query is exactly $\frac{1}{2}$ even after the $i$th round.

This concludes our proof of $Pr[\pred{win}^{\adv, \param,C,D}_{\pred{SQ}}]\leq \frac{1}{2} + \pred{negl}(\param)$.
\end{proof}


%\noindent
\subsubsection{\ECPLA Security Definition}
As we have shown that \dt is
\SQECPLA secure, using that result we
will now show that \dt is also \ECPLA secure. 
The \ECPLA game is played between two parties: the cloud-service
provider who is a ppt \emph{adversary} (denoted by
\adv) and a challenger (denoted by \cl) who is the client or
the owner of the plaintext audit log. The \ECPLA game is
played for any large enough security
parameter $\param$, for any predicate set $\mathbb{P}$, 
for any privacy policy \policy for which there exists $\inp$ 
 and \mymap such that $\inp\nsat\policy: \mymap$ holds. The game proceeds as
follows:
\begin{enumerate}
\item \cl generates an encryption key set \keys based on $\param$, 
$\mathbb{P}$, \cS, and the keying scheme $\mymap\cup\mathcal{A}$ (see Section~\ref{section:det} for description of $\mathcal{A}$) . 
$\keys\overset{\$}{\leftarrow} \pred{KeyGen}^\pred{DET}(1^{\param}, \mathbb{P}, \cS, \mymap\cup\mathcal{A})$.

\item \cl randomly chooses a bit $b$. $b\overset{\$}{\leftarrow}\{0, 1\}$.

\item \cl sends the policy \policy and the database schema \cS to \adv.

\item \cl sends $C$, $D$, the encryption of $C$ with keys corresponding to columns in which $C$ appears, and 
the encryption of $D$ with key $K_\pred{time}$ 
where $C=\pred{getConstant}(\policy)$ and $D=\pred{getTimeOffsetConst}(\policy)$
to  \adv. The function $\pred{getConstant}(\cdot)$ takes as
input a formula \policy and returns a set containing all the constants appearing in \policy.
The function $\pred{getTimeOffsetConst}(\cdot)$ takes as input a formula \policy and returns
a set containing all the time offset constants appearing in \policy. 

\item \adv chooses two plaintext audit logs $\cL_{0}$ and
$\cL_{1}$ with  schema \cS and $\cL_0 \neq \cL_1$, and sends it to \cl.

\item \cl encrypts $\cL_{b}$ to obtain the
encrypted audit log $e\cL_{b}=\langle e\dbd{b}, e\cT_{b}\rangle$, 
$e\cL_{b}\leftarrow\pred{EncryptLog}^\pred{DET}(\cL_b,\cS,\keys)$. 

\item \cl encrypts the constants in the policy \policy to obtain a constant-encrypted policy $\policy_e$ 
and shares with \adv. $\policy_e\leftarrow\pred{EncryptPolicyConstants}^\pred{DET}(\policy,\keys)$. 

\item \cl runs the \ereduce algorithm over the encrypted log $e\cL_b$ and the policy $\policy_e$,
$\ereduce(e\cL^b_i, \policy_e, \emptyset, \bullet)\Downarrow \langle\Sigma, \psi, cT\rangle$. 
Here, $\bullet$ represents the \emph{identity} substitution. 


\item \cl then sends $e\cL^{b}_{i}$, $\psi$, $\Sigma$, and $cT$ to \adv.
\item \adv finally outputs his guess bit $b'$.
\end{enumerate}
\adv wins the above \ECPLA game if 
$b=b'$, \adv does not ask for the encryption of a non-constant value in either 
of the domain, and $\cL_0\equiv_{(C,D)}\cL_1$. 
Let us denote the random variable indicating the success of \adv winning the above \ECPLA game by
$\pred{win}^{\adv, \param, \policy}$.

\begin{definition}[\ECPLA: Indistinguishability under equivalent chosen-plaintext log attack]
Any encrypted auditing framework is \ECPLA secure iff for all ppt adversary \adv, for all predicates $\mathbb{P}$, 
all privacy policy \policy, and all sufficiently large security parameter $\param$,
$Pr[\pred{win}^{\adv, \param, \policy}]\leq \frac{1}{2} + \pred{negl}(\param)$.
\end{definition}

We now have the following theorem which states that \dt is \ECPLA-secure. 
\begin{theorem}
\dt is \ECPLA secure.
\end{theorem}



\subsubsection{$\ECPLA^\pred{KH}$ Security Definition}
We will now show that the \kh has the $\ECPLA^\pred{KH}$ security 
based on the proof of \dt has the \ECPLA security. 
The $\ECPLA^\pred{KH}$ game is played between two parties: the cloud-service
provider who is a ppt \emph{adversary} (denoted by
\adv) and a challenger (denoted by \cl) who is the client or
the owner of the plaintext audit log. The $\ECPLA^\pred{KH}$ game is
played for any large enough security
parameter $\param$, 
for any database schema \cS, 
for any predicate set $\mathbb{P}$, and   
for any privacy policy \policy for which there exists $\inp$ 
 and \mymap such that $\inp\nsat\policy: \mymap$ holds. The game proceeds as
follows:
\begin{enumerate}
%\item The challenger obtains the database schema \cS from \policy. 


\item \cl generates an encryption key set \keys based on $\param$, $\mathbb{P}$, keying scheme $\mathcal{A}$ (see Section~\ref{section:kh} for description of $\mathcal{A}$) 
and 
the database schema \cS. 
$\keys\overset{\$}{\leftarrow} \pred{KeyGen}^\pred{KH}(1^{\param}, \mathbb{P}, \cS, \mathcal{A})$.


\item \cl randomly chooses a bit $b$,
$b\overset{\$}{\leftarrow}\{0, 1\}$.

\item \cl generates the token list $\vec{\Delta}$ based on \mymap, \cS, \param, and 
 \keys. $\vec{\Delta}\leftarrow \pred{GenerateToken}(1^\param,\cS,\mymap,\keys)$. 

\item \cl encrypts the constant of \policy to obtain a constant-encrypted policy $\policy_e$. 
$\policy_e\leftarrow\pred{EncryptPolicyConstants}^\pred{KH}(\policy,\keys)$.  

\item \cl sends the policies \policy and $\policy_e$, the database schema \cS, and $\vec{\Delta}$ to \adv.

\item \cl sends $C$, $D$, the encryption of $C$ with keys corresponding to columns in which $C$ appears, and 
the encryption of $D$ with key $K_\pred{time}$. 

\item \adv chooses two plaintext audit logs $\cL_{0}$ and
$\cL_{1}$ with schema \cS such that $\cL_0\neq \cL_1$, and sends it to \cl.

\item \cl encrypts the log $\cL_{b}$ to obtain the
encrypted audit log $e\cL_{b}=\langle e\dbd{b}, e\cT_{b}\rangle$, 
$e\cL_{b}\leftarrow\pred{EncryptLog}^\pred{KH}(\cL_b,\cS,\keys)$. 

\item \cl runs the \ereduce algorithm over the encrypted log $e\cL_b$,
$\ereduce(e\cL^b_i, \policy_e, \vec{\Delta}, \bullet)\Downarrow \langle\Sigma, \psi, cT\rangle$
\item \cl then sends $e\cL^{b}_{i}$, $\psi$, $\Sigma$, and $cT$ to \adv.
\item \adv finally outputs his guess bit $b'$.
\end{enumerate}

\adv wins the above $\ECPLA^\pred{KH}$ game if 
$b=b'$, \adv does not ask for the encryption of a non-constant value in either 
of the domain,  and $\cL_0\equiv_{(C,D)}\cL_1$. 
Let us denote the random variable indicating the success of the adversary \adv winning the above $\ECPLA^\pred{KH}$ game by
$\pred{win}^{\adv, \param, \policy}$.

\begin{definition}[$\ECPLA^\pred{KH}$: Indistinguishability under equivalent chosen-plaintext log attack with keyed hash]
Any encrypted auditing framework is $\ECPLA^\pred{KH}$ secure if and only if for all ppt adversary \adv, for all predicate set $\mathbb{P}$, 
all privacy policy \policy, for all database schema \cS, and all sufficiently large security parameter $\param$,
$Pr[\pred{win}^{\adv, \param, \policy}]\leq \frac{1}{2} + \pred{negl}(\param)$.
\end{definition}

\begin{theorem}
\kh is $\ECPLA^\pred{KH}$ secure.
\end{theorem}

\begin{proof}
The proof follows by the transitivity of the hybrid argument and 
the security of ADJ-JOIN keyed hash scheme~\cite{ADJJOIN}. It is easy to see that instead of giving the transfer keys $\vec{\Delta}$ if we 
generate the keys according to the keying scheme $\mymap\cup\mathcal{A}$ and also 
deterministically encrypt the log according to the keying scheme $\mymap\cup\mathcal{A}$, the $\ECPLA^\pred{KH}$ game gets translated to the \ECPLA game. 
By the proof of \ECPLA and by hybrid argument, 
we can say that \adv's advantage of winning the $\ECPLA^\pred{KH}$ game is exactly $\frac{1}{2}+\pred{negl}(\param)$. 
\end{proof}

\noindent
\textbf{Dummy Logs:}
We now explain the intuition behind our definition of the plaintext log equivalence
%between two plaintext audit logs 
 and its implication. Based on that intuition we show how
to generate a plaintext dummy audit log $\cL_d$ provided that we are given another
plaintext audit log $\cL$ such that $\cL_d\equiv_{(C,D)}\cL$ for some set
of constants $C$ and some well-formed set of distances $D$.

The intuition behind our equivalence definition between two plaintext audit logs is that
if we consistently replace each value  of the first audit log \cL with another dummy
value of the same length \emph{not in the domain of} \cL (with special care given to replacing the time stamps and replacing the constants in set $C$),
then if we run
our compliance checking algorithm over either of the plaintext audit log,
the resulting execution and the result of compliance checking algorithm will
look indistinguishable if we do not consider the concrete values involved.
For instance, if we have an entry in the first audit log saying
$\pred{send}(\pred{Alice}, \pred{Carol}, M_1)$ (\ie, \pred{Alice} is sending the message $M_1$ to
\pred{Carol}). We can replace all occurrences of \pred{Alice} in the audit log with another
dummy individual \pred{Carol} without
making  the execution of the algorithm distinguishable (not
considering the concrete values). Note that, we are emphasizing that
concrete values should not be considered as
when we encrypt the values in the audit log the adversary cannot tell whether certain
ciphertext is the encryption of either \pred{Alice} or \pred{Carol}.

Note that, we also emphasized that special care be taken while replacing
time-stamps and constants in the set $C$. We will first clarify how to replace
time-stamps. If we take two time stamps $t_1$ and $t_2$ from the original
plaintext audit log and they maintain the following relation: $t_1 + d_i \leq t_2 + d_j$ for
some $d_i, d_j\in D$. If we replace $t_1$ and $t_2$ with dummy time stamps $t^{dm}_1$ and
$t^{dm}_2$, respectively, to make the execution of the algorithm indistinguishable,
we have to ensure that the following relation also holds for $t^{dm}_1$ and
$t^{dm}_2$, that is $t^{dm}_1 + d_i \leq t^{dm}_2 + d_j$. One possible way to replace time
stamps is thus shift all the original time stamps with a constant offset.

About the constants in set $C$, we should not replace them with a dummy value
instead we should just copy them as it is in the dummy log.
In our setting, the adversary knows the plaintext constants in the set $C$
and also their encryption. Because we use
deterministic encryption, if one log has the constants and the other does not, then
the adversary can easily differentiate between the original and the dummy log.

It is straightforward to prove that: given any plaintext log $\cL$, a set of constants $C$,
and a well-formed set of distances $D$, if we create
a dummy log $\cL_d$ according to the approach described above, then $\cL\equiv_{(C,D)} \cL_d$.
Using this result and combining the result that \detkh has \ECPLA security,
we can prove that \detkh has ``real-versus-random'' type of security. The game will be
exactly like the \ECPLA game with one exception. Instead of the adversary choosing
a pair of equivalent plaintext audit logs, the adversary would now choose one plaintext
audit log and we randomly choose either to encrypt and run the compliance checking
algorithm on the audit log selected by the adversary or the dummy log we created
from the real log. The adversary wins if she can guess which audit log (real or dummy)
was encrypted. 

